Monitoring Collective Communication Among GPUs

Communication among devices in multi-GPU systems plays an important role in terms of performance and scalability. In order to optimize an application, programmers need to know the type and amount of the communication happening among GPUs. Although there are prior works to gather this information in MPI applications on distributed systems and multi-threaded applications on shared memory systems, there is no tool that identifies communication among GPUs. Our prior work, ComScribe, presents a point-to-point (P2P) communication detection tool for GPUs sharing a common host. In this work, we extend ComScribe to identify communication among GPUs for collective and P2P communication primitives in NVIDIA's NCCL library. In addition to P2P communications, collective communications are commonly used in HPC and AI workloads thus it is important to monitor the induced data movement due to collectives. Our tool extracts the size and the frequency of data transfers in an application and visualizes them as a communication matrix. To demonstrate the tool in action, we present communication matrices and some statistics for two applications coming from machine translation and image classification domains.

==> types_of_comm.tex <==
% !TEX root =  ./main.tex
\section{Communication Types}
\label{sec:typeComm}
\vspace{-0.2cm}
\subsection{Host-Device Communication}
In CUDA programming, a memory transfer between a host and a device can be realized in two ways: explicit transfer and implicit transfer. Explicit transfer refers to the \texttt{cudaMemcpy} or \texttt{cudaMemcpyAsync} function in CUDA Runtime API where the programmer can explicitly specify the kind (Host-to-Device, Device-to-Host, or cudaMemcpyDefault) of the memory transfer. Implicit transfer types are zero-copy memory and unified memory. Zero-copy memory paradigm allows a GPU to directly access host memory over PCIe or NVLink interconnect by pinning a memory region in host memory and mapping it to the GPU. A memory region allocated with unified memory via \texttt{cudaMallocManaged} is accessible from any processor (CPU or GPU) in the system. Page faults are handled by the page migration engine automatically. 
\vspace{-0.2cm}
\subsection{Peer-to-Peer (P2P) Communication}
A data transfer between two GPUs that support P2P memory access is considered as P2P communication. As in host-device communication, there are two types of a data transfer: explicit transfer and implicit transfer. In explicit transfer, the programmer can use either \texttt{cudaMemcpy} or \texttt{cudaMemcpyPeer}. If peer access is disabled, the data will be copied to the host and then transferred to the destination device. In P2P communication, implicit transfer types are also zero-copy memory and unified memory. In zero-copy memory, devices with peer access capability can read and write to each others’ memory through the data pointer. In unified memory, any memory region allocated with \texttt{cudaMallocManaged} can be accessed by the peer GPUs.   

\subsection{Collective Communication}
% \begin{figure}[ht]
%   \includegraphics[width=\textwidth]{figures/collectives.png}
%   \caption{Contents of each GPU's buffer before and after the collective operation in a four GPU setting.}
%   \label{fig:collectives}
% \end{figure}
Collective communication involve a data transfer between more than one GPU, unlike P2P communication where there is only one sender and receiver. In order to use a collective primitive on a group of GPUs (i.e. in a communicator), each GPU within the communicator is assigned a zero-based rank and each rank involved in a collective communication must call the same communication primitive function with compatible arguments. For example, they must be in the same communicator. 

NCCL provides five collective communication primitives: AllReduce, Broadcast, Reduce, AllGather, and Reduce-Scatter. Especially, AllReduce is frequently used in deep learning applications to share the local gradients. The  functionality of each collective primitive is described below:  
\vspace{-0.2cm}
\subsubsection{Broadcast:}
The broadcast collective involves the copying of data that resides in the root rank's memory to the all other rank's memory. 
\vspace{-0.2cm}
\subsubsection{Reduce:}
The Reduce collective is performing a reduction operation on data (e.g. sum, max) aggregated from all ranks in a communicator and writes the result in the specified rank's memory.
\vspace{-0.2cm}
\subsubsection{Reduce-Scatter}
The ReduceScatter collective performs the same operation as the Reduce operation, except the result is scattered in equal blocks among ranks, each rank getting a chunk of data based on its rank index. 
\vspace{-0.2cm}
\subsubsection{All-Gather}
In AllGather, each rank in the communicator aggregates N values from every rank into an output buffer. The output is ordered by rank index.
\vspace{-0.2cm}
\subsubsection{All-Reduce}
The All-Reduce collective is similar to Reduce collective. The only functional difference is that the result of the reduction is written into each rank's memory in the communicator instead of one rank. All-Reduce is a rank agnostic operation, i.e. reordering of ranks does not affect the outcome since all ranks will have identical data at the end. This operation is functionally equivalent to a reduce followed by a broadcast.

\begin{figure}[t]
\begin{center}
  \includegraphics[width=0.8\textwidth]{figures/allreduce_horizontal.png}
  \end{center}
  \caption{AllReduce: each rank receives the reduction of input values [cite]}
  \label{fig:workflow}
\vspace{-0.5cm}
\end{figure}

% \begin{table}[h!]
% \centering
%  \begin{tabular}{|c | c | c | c |} 
%  \hline
%  Col1 & Col2 & Col2 & Col3 \\ [0.5ex] 
%  \hline
%  1 & 6 & 87837 & 787 \\ 
%  \hline
%  2 & 7 & 78 & 5415 \\
%  \hline
%  3 & 545 & 778 & 7507 \\
%  \hline
%  4 & 545 & 18744 & 7560 \\
%  \hline
%  5 & 88 & 788 & 6344 \\ [1ex] 
%  \hline
%  \end{tabular}
% \end{table}
